Testing Halfspaces over Rotation-Invariant Distributions

We present an algorithm for testing halfspaces over arbitrary, unknown rotation-invariant distributions. Using $\tilde O(\sqrt{n}\epsilon^{-7})$ random examples of an unknown function $f$, the algorithm determines with high probability whether $f$ is of the form $f(x) = sign(\sum_i w_ix_i-t)$ or is $\epsilon$-far from all such functions. This sample size is significantly smaller than the well-known requirement of $\Omega(n)$ samples for learning halfspaces, and known lower bounds imply that our sample size is optimal (in its dependence on $n$) up to logarithmic factors. The algorithm is distribution-free in the sense that it requires no knowledge of the distribution aside from the promise of rotation invariance. To prove the correctness of this algorithm we present a theorem relating the distance between a function and a halfspace to the distance between their centers of mass, that applies to arbitrary distributions.

==> header.tex <==

%\usepackage{wrapfig}
%\usepackage[section]{placeins}
%\usepackage{float}


\usepackage[letterpaper, portrait, margin=1in]{geometry}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{url}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{mathtools}
\usepackage{parskip}
\usepackage{xspace}
\usepackage{verbatim}
\usepackage{mathrsfs}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage{pgf}
\usepackage{tikz}
\usepackage{tikz-qtree} % for drawing trees
\usepackage[dvipsnames]{xcolor}
\usepackage{todo}

%-------------------------------------------------------------------------------
% TikZ
%-------------------------------------------------------------------------------
\usetikzlibrary{intersections}

%-------------------------------------------------------------------------------
% Fonts
%-------------------------------------------------------------------------------
%\usepackage[math]{iwona}
%\usepackage{fourier}
%\usepackage{cmbright}
%\usepackage[T1]{fontenc}
%\usepackage{pifont}

%\usepackage{bbm}
\usepackage{dsfont}

\newcommand{\cmark}{\ding{51}}
%\newcommand{\xmark}{\ding{55}}
\newcommand{\xmark}{}

%-------------------------------------------------------------------------------
% Theorems
%-------------------------------------------------------------------------------
\topsep=1em % spacing between plain theorems
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{question}[theorem]{Question}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

%-------------------------------------------------------------------------------
% Environments
%-------------------------------------------------------------------------------

% environment combining equation and aligned
\newenvironment{eqalign}
{\begin{equation}\begin{aligned}}
{\end{aligned}\end{equation}}


\newcommand{\ignore}[1]{}


%-------------------------------------------------------------------------------
% Complexity Classes
%-------------------------------------------------------------------------------
\newcommand{\NP}{\textsf{NP}}

%-------------------------------------------------------------------------------
% Common functions
%-------------------------------------------------------------------------------
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\supp}{supp}   % support
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\trunc}{trunc}
\DeclareMathOperator{\Tr}{Tr}       % trace
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\Margin}{margin}

\newcommand{\HatCom}{\widehat{\mathsf{Com}}}
\newcommand{\Com}[1]{\mathsf{Com}\left( #1 \right)}
%\newcommand{\dist}[1]{\mathsf{dist}\left( #1 \right)}
\newcommand{\dist}{\mathsf{dist}}
\newcommand{\err}{\mathsf{err}}

\DeclareMathOperator{\Argmin}{argmin}
\newcommand{\argmin}{\Argmin\limits}

\DeclareMathOperator{\Argmax}{argmax}
\newcommand{\argmax}{\Argmax\limits}

\newcommand{\acos}{\cos^{-1}}
\newcommand{\asin}{\sin^{-1}}

\newcommand{\VCdim}[1]{\mathsf{VC}\left( #1 \right)}

\newcommand{\opt}{\mathsf{opt}}

% Probability stuff

% Variance:
\DeclareMathOperator{\Cov}{Cov}
%\newcommand{\Var}[1]{\bV \left[ #1 \right]}
\newcommand{\Var}[1]{\mathrm{Var} \left[ #1 \right]}
\newcommand{\Varu}[2]{\underset{ #1 } \bV \left[ #2 \right]}
\newcommand{\Varuc}[3]{\underset{ #1 } \bV \left[ #2 \;\; \left\mid \;\; #3 \right. \right]}


% Expectation:
\newcommand{\Ex}[1]{\bE \left[ #1 \right]}
\newcommand{\Exu}[2]{\underset{#1} \bE \left[ #2 \right] }
\newcommand{\Exuc}[3]{\underset{#1} \bE \left[ #2 \;\; \left| \;\; #3
\right.\right] }

% Probability:
\renewcommand{\Pr}[1]{\bP \left[ #1 \right]} % Probability
\newcommand{\Pru}[2]{\underset{ #1 }\bP \left[ #2 \right]}
\newcommand{\Pruc}[3]{\underset{ #1 }\bP \left[ #2 \;\; \mid \;\; #3 \right]}

% Influence:
\DeclareMathOperator{\Inf}{Inf}

% Stability:
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\NS}{NS}

% Complexity stuff
\newcommand{\BigO}[1]{O \left( #1 \right) }
\newcommand{\SmallO}[1]{\mathcal{o} \left( #1 \right)}
\newcommand{\BigOmega}[1]{ \Omega \left( #1 \right) }
\newcommand{\SmallOmega}[1]{ \omega \left( #1 \right) }
\newcommand{\BigTheta}[1]{\Theta \left( #1 \right) }

%-------------------------------------------------------------------------------
% Common symbols
%-------------------------------------------------------------------------------
\newcommand{\define}{\vcentcolon=}

% exponential function
\renewcommand{\exp}[1]{\mathrm{exp}\left( #1 \right)}

% floor and ceiling
\newcommand{\floor}[1]{\ensuremath{\lfloor #1 \rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\lceil #1 \rceil}}

% norm
%\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\norm}[1]{\| #1 \|}

% under bar
\newcommand{\ubar}[1]{\underline{#1}}

% bracket fraction
\newcommand{\fracb}[2]{\left( \frac{#1}{#2} \right)}

% inline matrix
\newcommand{\imatrix}[1]{\left[ \begin{smallmatrix} #1 \end{smallmatrix} \right]}

% "consistency" binary operator
\newcommand{\cons}{\triangleleft}
\newcommand{\snoc}{\triangleright}

\newcommand{\ket}[1]{\ensuremath{\left| {#1} \right\rangle}}
\newcommand{\bra}[1]{\ensuremath{\left\langle {#1} \right|}}

%\newcommand{\inn}[1]{\left\langle #1 \right\rangle}
\newcommand{\inn}[1]{\langle #1 \rangle}
\newcommand{\inner}[2]{\ensuremath{\langle{#1}|{#2}\rangle}}

%\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\abs}[1]{| #1 |}

% indicator or identity functions
\newcommand{\id}{\ensuremath{\mathds{1}}}

% indicator
\newcommand{\ind}[1]{\mathds{1} \left[ #1 \right] }

\newcommand{\nth}[1]{\ensuremath{#1^{\textup{th}}}}

% derivatives
\newcommand{\partiald}[2]{\frac{\partial #1}{\partial #2}}

%-------------------------------------------------------------------------------
% Common sets
%-------------------------------------------------------------------------------
\newcommand{\complex}{\mathbb C}
\newcommand{\integers}{\mathcal{N}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\pmset}{\{\pm 1\}}

%-------------------------------------------------------------------------------
% Text shortcuts
%-------------------------------------------------------------------------------
\newcommand{\x}[1]{\text{#1}}
\newcommand{\xh}[1]{\hspace{2em}\text{#1}}
\renewcommand{\sc}{\textsc}
\renewcommand{\it}{\textit}
\renewcommand{\bf}{\textbf}
\renewcommand{\cal}{\mathcal}

%-------------------------------------------------------------------------------
% Special formatting
%-------------------------------------------------------------------------------

% circled letters
\newcommand\encircle[1]{%
  \tikz[baseline=(X.base)]
    \node (X) [draw, shape=circle, inner sep=0] {\strut #1};}

%-------------------------------------------------------------------------------
% Comments and notes
%-------------------------------------------------------------------------------
\newcommand{\note}[1]{{\color{Brown} \;\ifmmode \text{#1} \else #1 \fi\;}}
\newcommand{\lnote}[1]{{\reversemarginpar \marginpar{\color{MidnightBlue} #1}}}
\newcommand{\rnote}[1]{\marginpar{\color{MidnightBlue} #1}}

%-------------------------------------------------------------------------------
% Shortcuts for special characters
%-------------------------------------------------------------------------------

% Calligraphic characters
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}

% Blackboard Bold characters
\newcommand{\bA}{\ensuremath{\mathbb{A}}}
\newcommand{\bB}{\ensuremath{\mathbb{B}}}
\newcommand{\bC}{\ensuremath{\mathbb{C}}}
\newcommand{\bD}{\ensuremath{\mathbb{D}}}
\newcommand{\bE}{\ensuremath{\mathbb{E}}}
\newcommand{\bF}{\ensuremath{\mathbb{F}}}
\newcommand{\bN}{\ensuremath{\mathbb{N}}}
\newcommand{\bP}{\ensuremath{\mathbb{P}}}
\newcommand{\bR}{\ensuremath{\mathbb{R}}}
\newcommand{\bS}{\ensuremath{\mathbb{S}}}
\newcommand{\bT}{\ensuremath{\mathbb{T}}}
\newcommand{\bV}{\ensuremath{\mathbb{V}}}
\newcommand{\bZ}{\ensuremath{\mathbb{Z}}}

